Exploring Anchor-based Detection for Ego4D Natural Language Query

In this paper we provide the technique report of Ego4D natural language query challenge in CVPR 2022. Natural language query task is challenging due to the requirement of comprehensive understanding of video contents. Most previous works address this task based on third-person view datasets while few research interest has been placed in the ego-centric view by far. Great progress has been made though, we notice that previous works can not adapt well to ego-centric view datasets e.g., Ego4D mainly because of two reasons: 1) most queries in Ego4D have a excessively small temporal duration (e.g., less than 5 seconds); 2) queries in Ego4D are faced with much more complex video understanding of long-term temporal orders. Considering these, we propose our solution of this challenge to solve the above issues.

==> relatedwork.tex <==
\section{Related Work}
Given a video and a natural language query, textguided
video temporal grounding aims to predict the starting and ending time of the video clip
that best matches the query sentence. Existing methods for this task can be categorized into two
groups, i.e., two-stage and one-stage schemes (see Figure 1(a)(b)). Most two-stage approaches adopt
a propose-and-rank pipeline, where they first generate clip proposals and then rank the proposals
based on their similarities with the query sentence. Early two-stage methods [10, 14] obtain proposals
by scanning the whole video with sliding windows. Since the sliding window mechanism
is computationally expensive and usually produces many redundant proposals, numerous methods
are subsequently proposed to improve the efficiency and effectiveness of proposal generation. The
TGN model [2] performs frame-by-word interactions and localize the proposals in one single pass.
Other approaches focus on reducing redundant proposals by generating query-guided proposals [31]
or semantic activity proposals [3]. The MAN method [34] models the temporal relationships between
proposals using a graph architecture to improve the quality of proposals. To alleviate the computation
of observing the whole video, reinforcement learning [13, 30] is utilized to guide the intelligent agent
to glance over the video in a discontinuous way. While the two-stage methods achieve promising
results, the computational cost is high for comparing all proposal-query pairs, and the performance is
largely limited by the quality of proposal generation.

